NewsComp: Facilitating Diverse News Reading through Comparative Annotation

To support efficient, balanced news consumption, merging articles from diverse sources into one, potentially through crowdsourcing, could alleviate some hurdles. However, the merging process could also impact annotators' attitudes towards the content. To test this theory, we propose comparative news annotation, i.e., annotating similarities and differences between a pair of articles. By developing and deploying NewsComp -- a prototype system -- we conducted a between-subjects experiment(N=109) to examine how users' annotations compare to experts', and how comparative annotation affects users' perceptions of article credibility and quality. We found that comparative annotation can marginally impact users' credibility perceptions in certain cases. While users' annotations were not on par with experts', they showed greater precision in finding similarities than in identifying disparate important statements. The comparison process led users to notice differences in information placement/depth, degree of factuality/opinion, and empathetic/inflammatory language use. We discuss implications for the design of future comparative annotation tasks.

==> tex/0commands.tex <==
\newcommand{\sys}{\textit{NewsComp}}
% NewsComp
% education, multi perspective
\newcommand{\sysfull}{Comparative News Annotation}
\newcommand{\papertitle}{NewsComp: Facilitating Diverse News Reading through Comparative Annotation}
% Balanced News Comprehension
% Comparative News Reading for Fun and Profit \s
% Probing News through a Comparative Lens
% Engaging Novice and Expert News Consumers with Opposing News Narratives via Comparison
% Pluralistic/Relativistic/Divergent News Consumption via Comparative Annotation
% Would Comparison Lead to Perception Correction? Exploring the Application of Comparative Annotation for Diverging News Consumption
% Probing News through a Comparative Lens 
% Probing the Application of Comparative Annotation for Diverging News Consumption


\newcommand{\rqt}[2]{\hspace{5pt} \textbf{RQ#1}. \textit{#2}}
\newcommand{\rqsub}[2]{\hspace{10pt} \textbf{#1}. \textit{#2}}

\newcommand{\qt}[2]{\begin{quote}\small{\textit{``#2''}} \hspace{5pt} --- \textbf{#1}\end{quote} }


\newcommand{\addition}[1]{\textcolor{black}{#1}}
\newcommand{\additionminor}[1]{\textcolor{black}{#1}}

\newcommand{\inlineqt}[2]{\textit{``#2''} - \textit{#1}}

\newcommand{\participants}{109}
\newcommand{\topics}{two}
\newcommand{\articlesperparticipant}{two}
\newcommand{\articles}{four}
\newcommand{\experts}{two}

\DeclareRobustCommand{\numone}{\includegraphics[scale=0.3]{figures/ot-interface-1.pdf}}
\DeclareRobustCommand{\numtwo}{\includegraphics[scale=0.3]{figures/ot-interface-2.pdf}}
\DeclareRobustCommand{\numthree}{\includegraphics[scale=0.3]{figures/ot-interface-3.pdf}}
\DeclareRobustCommand{\numfour}{\includegraphics[scale=0.3]{figures/ot-interface-4.pdf}}
\DeclareRobustCommand{\numfive}{\includegraphics[scale=0.3]{figures/ot-interface-5.pdf}}
\DeclareRobustCommand{\numsix}{\includegraphics[scale=0.3]{figures/ot-interface-6.pdf}}

\DeclareRobustCommand{\arrowsolid}{\includegraphics[scale=0.03]{figures/solid_arrow.png}}

\DeclareRobustCommand{\arrowdashed}{\includegraphics[scale=0.03]{figures/dashed_arrow.png}}

\DeclareRobustCommand{\arrowanim}{\animategraphics[autoplay,loop,scale=0.03]{1}{figures/arrow-}{0}{1}}



\newcommand{\rqone}{How well do users perform comparative annotation?}

\newcommand{\rqtwo}{How does comparative news annotation affect users' perceptions of credibility and news quality?}

==> tex/1abstract.tex <==
% high-level vision version
\begin{abstract}
% Despite the multitude of choices to consume news online, it is challenging to critically compare and comprehend diverse perspectives.
\addition{To support efficient, balanced news consumption, merging articles from diverse sources into one, potentially through crowdsourcing, could alleviate some hurdles.
However, the merging process could also impact annotators' attitudes towards the content.}
To test this theory, we propose comparative news annotation; that is, annotating similarities and differences between a pair of articles.
By developing and deploying \sys{}---a prototype system---we conducted a between-subjects experiment (N~=~\participants) to examine how users' annotations compare to experts', and how comparative annotation affects users' perceptions of article credibility and quality.
We found that comparative annotation can marginally impact users' credibility perceptions in certain cases; it does not impact perceptions of quality.
While users' annotations were not on par with experts', they showed greater precision in finding similarities than in identifying disparate important statements.
\addition{The comparison process also led users to notice differences in information placement and depth, degree of factuality/opinion, and empathetic/inflammatory language use.}
\addition{We discuss implications for the design of future comparative annotation tasks.}
% Overall, our study has implications for the design of future multiperspective news reading systems.
% This idea allows (i) annotators to engage and read news articles on a single topic from diverse sources, and (ii) provides annotation useful to merge multiple stories.
\end{abstract}
%Our analysis showed poor annotation performance by participants.
%However, certain information can differentiate incorrect annotations, e.g., the number of users annotating an item or the rationale behind an annotation.
% We further found that comparative annotation can marginally impact users' credibility perception in certain cases.

% Despite having a multitude of choices to consume news online, users tend to encamp themselves towards one-sided narratives, further restrained by
% We analyzed how users news expertise and annotation rational relate to correct and incorrect annotations.
% Our results reveal that the annotation group's credibility ratings get closer to expert ratings for certain article pair.
% Furthermore, users with lower news expertise made both more accurate annotations and more false positives.

% We conducted a user study to test whether engagement through an annotation task affects users' perception on articles.

% \textit{What if users could simultaneously compare, annotate and consume content from diverse sources?}
% The goal of this work is to explore how to engage users with diverse perspectives on a news item.
% better credibility assessment. 
% news quality assessment 
% getting close to experts (increased media literacy?) 
% However, it is challenging for news readers to critically comprehend and compare opposing perspectives from diverse sources. 

% In this work, we explore this concept through the design of a comparative news annotation interface.
%We began by examining whether providing existing (algorithm-generated) annotations would improve user engagement and found scant evidence.

% previous version
% \begin{abstract}
% To counter polarization, liberal democratic principle suggests that people should engage with news from politically diverse sources.
% In this work, we explore the application of comparative news annotation interfaces for such purpose through a series of think-aloud interviews and a between-subject experiment. 
% Through the interviews, we find that when users browse a pair of news articles with existing (algorithm-generated) statement similarity annotation, they pay less attention to such annotations.
% In a between-subject experiment(n=\participants) with two pairs (low-/high-similarity) of news articles, we test whether promoting engagement through annotation affects users' perception on articles and how user characteristics affect annotation performance. 
% Our analysis reveal that treatment users' credibility rating error was significantly lower on article-pair with low similarity compared to the control users'.
% Furthermore, users with low news-expertise  made more correct annotations compared to high-expertise counterparts, at the cost of making more errors.
% Overall, our study has implications for designing future comparative content annotation systems.
% \end{abstract}
% if anyone can squeeze the next line somehow, it would be great 
% We find users mostly find similarity by content (rarely by themes) while finding statements with certain clarifications, elaboration and missing information to be important to include in the other articles of the pair. 



% , a task requiring extra time and effort.
% and more on finding controversy
% (elaboration or condensation,) 
% connotation similarity.
% For content where they are not similar, users hardly mostly skip over them with few analyzing importance, partisanship/perspective.

% 1) How can we design interface for comparative news reading? 
% In the study, we used two pairs of news articles on two contentious topics while varying the degree of similarities within a pair and collected the ground truths labels for them from \experts{} experts.
% where users have to engage with content by performing the annotations themselves. Here we ask:
% i) \rqone{} and,
% ii) \rqtwo{}

% We conducted the experiment with two pairs of news articles (low vs high similarity) where treatment users read and annotate a pair of news articles compared to control users only reading one of the pair.

